MCTS with Refinement for Proposals Selection Games in Scene Understanding

We propose a novel method applicable in many scene understanding problems that adapts the Monte Carlo Tree Search (MCTS) algorithm, originally designed to learn to play games of high-state complexity. From a generated pool of proposals, our method jointly selects and optimizes proposals that minimize the objective term. In our first application for floor plan reconstruction from point clouds, our method selects and refines the room proposals, modelled as 2D polygons, by optimizing on an objective function combining the fitness as predicted by a deep network and regularizing terms on the room shapes. We also introduce a novel differentiable method for rendering the polygonal shapes of these proposals. Our evaluations on the recent and challenging Structured3D and Floor-SP datasets show significant improvements over the state-of-the-art, without imposing hard constraints nor assumptions on the floor plan configurations. In our second application, we extend our approach to reconstruct general 3D room layouts from a color image and obtain accurate room layouts. We also show that our differentiable renderer can easily be extended for rendering 3D planar polygons and polygon embeddings. Our method shows high performance on the Matterport3D-Layout dataset, without introducing hard constraints on room layout configurations.

==> A_Limitations.tex <==
\section{Limitations and Future Work}

We demonstrate some failure cases of MonteFloor in Figure~\ref{fig:fails}. Even though our method achieves state-of-the-art results on existing datasets we do believe there is still a large potential for improvements:
\begin{itemize}
    \item The number of vertices of polygonal proposals is determined strictly by the polygonized outputs of the masks from Mask R-CNN. It would be interesting to consider possibility of dynamically adding, or removing, vertices of polygonal proposals. Similarly, it would be interesting to dynamically generate new rooms in places where large discrepancies are detected.
    
    \item Density maps are a useful representation, but in practice, they can still be ambiguous in some cases. Hence, considering additional information such as perspective views, and camera trajectory, could be very helpful to deal with such ambiguities.  
    
    
    \item In general proposals selection games it is clear from initialization that some proposals are unlikely to be part of the final solution. Using prior information about the quality of proposals to initialize node scores in the tree could make our approach run even faster.
\end{itemize}


\newlength{\suppbadresultwidth}
\setlength{\suppbadresultwidth}{0.3\linewidth}
\newcommand{\suppbaderesult}[1]{
\includegraphics[width=\suppbadresultwidth]{supp_figures/s3d_qual/#1_density.png} & 
\includegraphics[width=\suppbadresultwidth]{supp_figures/s3d_qual/#1_fsp.png} &
\includegraphics[width=\suppbadresultwidth]{supp_figures/s3d_qual/#1_ours_edit.png} &
\includegraphics[width=\suppbadresultwidth]{supp_figures/s3d_qual/#1_gt.png} \\}
\begin{figure*}
    \centering
    \begin{tabular}{cccc}
    \suppbaderesult{scene_03250}
    \suppbaderesult{scene_03258}
    \suppbaderesult{scene_03310}
    Density Map & Floor-SP & MonteFloor (Ours) & Ground Truth \\
    \end{tabular}    \caption{Failure Cases. First row, red arrow: Our reconstruction of the green room is incorrect as there are some ambiguities in the density map for this region. In contrast, Floor-SP is more likely to produce Manhattan layouts in such situations. Second row, red arrow: None of the generated polygonal proposals for the pink room are adequate to represent the actual shape. Floor-SP performs graph-based search on pixel-locations that lie on the polygonal curve. As the final polygon is generated after the search, they obtain better reconstruction in this example. Third row, red arrow: Similarly to Floor-SP, we were not able to remove false positive proposal. This implies that the metric network could be further improved.}
    \label{fig:fails}
\end{figure*}

==> A_MCTSwithRef.tex <==
\newcommand{\UCB}{{UCB}}
\newcommand{\opt}{{opt}}

%% \newcommand{\ScoreSum}{\text{ScoreSum}}
\newcommand{\Score}{\text{Score}}
\newcommand{\priorScore}{\text{fitness}}
\newcommand{\explC}{k_\text{expl}}
\newcommand{\globalScore}{Score}
% \newcommand{\calC}{\mathcal{C}}
% \newcommand{\calChildren}{\text{children}}
% \newcommand{\calN}{\mathcal{N}}
% \newcommand{\calCC} {\text{children}}
% \newcommand{\calCC} {\mathcal{C} }

\newcommand{\fn}[1]{\textsc{#1}}
\newcommand{\Each}{ \textbf{each}\xspace}
\newcommand{\return}{ \textbf{return}\xspace}

\newcommand{\anchor}{\text{anchor}}
\newcommand{\comp}{\text{comp}}
\newcommand{\curr}{\text{curr}}
\newcommand{\incomp}{\text{incomp}}
\newcommand{\pool}{\text{pool}}
\newcommand{\Root}{\text{root}}


\section{MCTS Implementation}

In this section, we provide more details about our implementation of Monte Carlo Tree Search~(MCTS) with our refinement step.

\textbf{Tree nodes.} As explained in the main paper, the nodes contain several attributes. Every node is associated with some proposal $P_i$, but the same proposal $P_i$ is associated with one or more nodes along different sub-paths of the tree. Every node $\calN$ also keeps track of its ``node score'' $Q(\calN)$ and number of visits $n(\calN)$ that will be used later to guide the search towards the  most promising directions. A node can have multiple children nodes $\calC(\calN)$ and has a single parent node.

\textbf{Initialization.} Initially, the search tree contains only a root node and is built online by expanding the tree in the most promising direction at every iteration.

During the search, we follow the standard Select-Expand-Simulate-Update strategy:

\textbf{Selection step.} At each iteration, and starting from the root node, we traverse existing nodes at each level of the tree by following the Upper Confidence Bound~(UCB) criterion: From current node $\calN_\curr$, we select its child node $\calN \in \calC(\calN_\curr)$ that maximizes the criterion
%
 \begin{align}
  \arg\max_{\calN \in \calC(\calN_\curr)} Q(\calN) +
  \lambda_\UCB \cdot \sqrt{\frac{\log n(\calN_{curr})}{n(\calN)}} \> ,
  \label{eq:UCB}
\end{align}
%
where $\lambda_\UCB$ is a hyperparameter that balances exploitation and the exploration during the search.

% \sinisarmk{This notation is from MCSS. Do we need to change it?}

\textbf{Expansion step.} If during selection, there is a node with a child node $\calN \in \calC(\calN_\curr)$ that has not been created yet, we do not follow the selection criterion, but instead, we add $\calN$ to the tree. We set $Q(\calN) = - \infty$ and $n(\calN) = 0$ at this stage.

\textbf{Simulation step.} Immediately after the expansion step, we perform a simulation step and randomly create and traverse the children nodes until we reach a leaf node of the tree. 

\textbf{Refinement step.} Whenever a leaf node is reached during simulation, we run 1 iteration of the Adam optimizer~\cite{kingma2014adam} on the selected proposals $P$ to minimize $\calL(P)$ (Eq.~(1) of the main paper) and calculate the score $S = -\calL(P)$:  
Running more iterations decreases the number of necessary MCTS iterations, but still results in longer run-times. Instead, we allow the tree search to select already visited solutions. This results in faster run-time and accurate solutions, as we will run multiple refinement steps on the most promising solutions, but few on the less likely ones.

\textbf{Update step.} Once we know the score $S$ for a set of proposals $P$ after the refinement step, for every traversed node $\calN$, we update the node score $Q(\calN) \leftarrow \max(Q(\calN), S)$ and increment $n(\calN)$.

During experiments, for each scene we set $\lambda_\UCB = 1$ initially, and linearly decay it such that the last MCTS iteration uses $\lambda_\UCB = 0.01$.

\subsection{Multiple Optimizers}

As the number of proposals increases, optimizer has to deal with much larger number of learning parameters. In turn, this leads to larger computation times during optimization step. To overcome this issue, we employ multiple optimizers: For each leaf node in the tree, we create an optimizer that optimizes the set of proposals along corresponding path in the tree. Such approach improves computation times considerably.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************

